A Hierarchical Aggregation Framework for Efficient Multilevel Visual Exploration and Analysis

Data exploration and visualization systems are of great importance in the Big Data era, in which the volume and heterogeneity of available information make it difficult for humans to manually explore and analyse data. Most traditional systems operate in an offline way, limited to accessing preprocessed (static) sets of data. They also restrict themselves to dealing with small dataset sizes, which can be easily handled with conventional techniques. However, the Big Data era has realized the availability of a great amount and variety of big datasets that are dynamic in nature; most of them offer API or query endpoints for online access, or the data is received in a stream fashion. Therefore, modern systems must address the challenge of on-the-fly scalable visualizations over large dynamic sets of data, offering efficient exploration techniques, as well as mechanisms for information abstraction and summarization. In this work, we present a generic model for personalized multilevel exploration and analysis over large dynamic sets of numeric and temporal data. Our model is built on top of a lightweight tree-based structure which can be efficiently constructed on-the-fly for a given set of data. This tree structure aggregates input objects into a hierarchical multiscale model. Considering different exploration scenarios over large datasets, the proposed model enables efficient multilevel exploration, offering incremental construction and prefetching via user interaction, and dynamic adaptation of the hierarchies based on user preferences. A thorough theoretical analysis is presented, illustrating the efficiency of the proposed model. The proposed model is realized in a web-based prototype tool, called SynopsViz that offers multilevel visual exploration and analysis over Linked Data datasets.

==> overview.tex <==
%!TEX root = main.tex

\section{Framework Overview}
\label{sec:over}
% \vspace{-3mm}

%\stitle{Hierarchical Model.}  
%{\color{red}{[na pume liga logia me pia logiki ftiaxnonte oi ierarchies ..kai ti
%vlepei o telikos xristis]. analoga me to edios tvn data - calsses, numeric,
%date time- pws ftiaxnoume ta groups}}

\eat{ 
\stitle{Hierarchical Model.}  
{\color{red}{
1)efficient statistics computation  using aggregation over levels 
2) interactive hierarchical model 
3) on-the-fly hierarchy construction (based on either data distribution or user's preferences)
4) overview and level-of-detail are defined based on either data distribution or user's preferences.
5)legacy visualization techniques can be transformed into hierarchical structures handling very large data. 
6) zoom on demand / details on demand 
7) ... 



The triples <subject, predicate, object> of each property that will be visualized are organized in clusters based on the value of their object. For instance,  in the case of numeric objects, triples can be included in clusters of the form [0, 10], [10, 20] i.e. triples with object value between 0-10 are included in the first cluster etc. These clusters can be clustered again to form an hierarchy.
The clusters can either have a fixed range of values or a fixed number of triples. The range of the clusters and the clustering of the previous level's clusters is computed based on the data distribution or the user's preferences.
For each property they have chosen to visualize, the users are presented with the top clusters of the hierarchy, thus gaining an overview of the data. Thus, they can chose the values range they wish to see in detail. For each cluster, statistics and sample data are presented helping the user can gain a better understanding of the data it contains. At the bottom of the hierarchy, the raw data (RDF triples) are presented in the appropriate chart (timeline for dates, column/line/area etc. for numbers).
}} 



\stitle{Hierarchical Construction.} .. 

\stitle{Statistics.} dataset stat / node stat 

\stitle{Metadata.} }

The architecture of \sviz is presented in Figure~\ref{fig:arch}.
Our scenario involves three main parts: the Client GUI, the  \sviz framework,
and the input data. The \textit{Client} part, corresponds to the framework's
front-end offering several functionalities to the end-users (e.g., statistical
analysis, facet search, etc.).
\sviz consumes RDF data as \textit{Input data}; optionally, OWL-RDF/S
vocabularies/ontologies describing the input data can be loaded.
 Next,  we describe the basic components of the \sviz  framework. 

In the preprocessing phase,  the \textit{Data and Schema Handler}
parses the input data and inferes schema information (e.g., properties domain(s)/range(s), class/property  hierarchy, type of
instances, type of properties, etc.).
\textit{Facets Generator} generates class and property facets over input data. 
%It exploits
%schema information and organizes triples into different facets - stored as
%separate named graphs - based on the types of classes and properties. This
%result to an efficient facets search mechanism, which uses precomputed groups of data.
\textit{Statistics Generator} computes several statistics regarding the
schema, instances and graph structure of the input dataset, such as the number
of different types of classes and properties, or the number of sameAs triples,
 or finally the average in/out degree of the RDF graph, respectively.
\textit{Metadata Extractor} collects dataset metadata which can be used for data quality assessment.
\textit{Hierarchical Model Module}
adopts our hierarchy model and stores the initial data enriched with the information computed during the preprocessing phase.


During runtime the following components are involved.
\textit{Hierarchy Specifier} is responsible for managing the
configuration parameters of our hierarchy model, e.g., the number of
hierarchy levels, the number of nodes per level, and providing this
information to the Hierarchy Constructor. 
\textit{Hierarchy Constructor}
implements the hierarchy model. 
Based on the selected facets, and the hierarchy configuration: 
 it determines the hierarchy of groups and the contained triples, and computes the 
statistics about their contents (e.g., range, variance, mean, number of triples contained, etc.).
\textit{Visualization Module} allows the interaction between the user and the framework, 
allowing several operations (e.g, navigation, filtering, hierarchy specification) over the visualized data.  


